FedDR -- Randomized Douglas-Rachford Splitting Algorithms for Nonconvex Federated Composite Optimization

We develop two new algorithms, called, FedDR and asyncFedDR, for solving a fundamental nonconvex composite optimization problem in federated learning. Our algorithms rely on a novel combination between a nonconvex Douglas-Rachford splitting method, randomized block-coordinate strategies, and asynchronous implementation. They can also handle convex regularizers. Unlike recent methods in the literature, e.g., FedSplit and FedPD, our algorithms update only a subset of users at each communication round, and possibly in an asynchronous manner, making them more practical. These new algorithms can handle statistical and system heterogeneity, which are the two main challenges in federated learning, while achieving the best known communication complexity. In fact, our new algorithms match the communication complexity lower bound up to a constant factor under standard assumptions. Our numerical experiments illustrate the advantages of our methods over existing algorithms on synthetic and real datasets.

==> conclusions.tex <==
\section{Conclusions}\label{sec:concl}
We have developed two novel FL algorithms by combining a nonconvex DR splitting scheme, a randomized block-coordinate strategy, and an asynchronous implementation.
Both algorithms achieve the state-of-the-art worst-case communication complexity under standard assumptions and have several advantages compared to existing methods.
Our second algorithm is asynchronous and works with a variety configurations.
Our numerical results show that our methods have competitive performance on both synthetic and real datasets over their competitors.

